Numerical analysis of a non-clamped dynamic thermoviscoelastic contact problem

In this work, we analyze a non-clamped dynamic viscoelastic contact problem involving thermal effect. The friction law is described by a non-monotone relation between the tangential stress and the tangential velocity. This leads to a system of second-order inclusion for displacement and a parabolic equation for temperature. We provide a fully discrete approximation of the problem and find optimal error estimates without any smallness assumption on the data. The theoretical result is illustrated by numerical simulations.

==> OLD/commands_old.tex <==
\newcommand{\norma}[1]{\|#1\|}
\newcommand{\nor}[2]{\|#1\|_{#2}}
\def\real{\mathbb{R}}
\def\nat{\mathbb{N}}
\def\interi{\mathbb{Z}}
\def\raz{\mathbb{Q}}
\def\arg{\text{arg}}
\def\Sd{\mbox{{\boldmath{${\mathbb S}$}}$^d$}}

%\newcommand{\norma}[1]{\|#1\|}
%\newcommand{\real}{\mathbb{R}}
\newcommand{\sd}{\mathbb{S}}
%\newcommand{\nat}{\mathbb{N}}
\newcommand{\G}{\Gamma}
\newcommand{\C}{\mathcal{C}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cH}{{\cal H}}
\newcommand{\tx}{\textstyle}
\newcommand{\Div}{\mbox{\rm Div\,}}

%\newcommand{\aktau}{A_{\tau}^k}
%\newcommand{\mktau}{M_{\tau}^k}
\newcommand{\etaktau}{\eta_{\tau}^k}
%\newcommand{\fktau}{f_{\tau}^k}
%\newcommand{\wktau}{w_{\tau}^k}
%\newcommand{\uktau}{u_{\tau}^k}
\newcommand{\zktau}{z_{\tau}^k}
%\newcommand{\xiktau}{\xi_{\tau}^k}

\newcommand{\wktau}{w_{\tau}^k}
\newcommand{\uktau}{u_{\tau}^k}

\newcommand{\xiktau}{\xi_{\tau}^k}
\newcommand{\fktau}{f_{\tau}^k}

\newcommand{\wktauminus}{w_{\tau}^{k-1}}
\newcommand{\uktauminus}{u_{\tau}^{k-1}}
\newcommand{\xiktauminus}{\xi_{\tau}^{k-1}}
\newcommand{\fktauminus}{f_{\tau}^{k-1}}

\newcommand{\witau}{w_{\tau}^i}
\newcommand{\uitau}{u_{\tau}^i}

\newcommand{\xiitau}{\xi_{\tau}^i}
\newcommand{\fitau}{f_{\tau}^i}

\newcommand{\witauminus}{w_{\tau}^{i-1}}
\newcommand{\uitauminus}{u_{\tau}^{i-1}}
\newcommand{\xiitauminus}{\xi_{\tau}^{i-1}}
\newcommand{\fitauminus}{f_{\tau}^{i-1}}


\newcommand{\itF}{\mbox{\boldmath{$F$}}}
\newcommand{\itg}{\mbox{\boldmath{$g$}}}
\newcommand{\bg}{\mbox{\boldmath{$g$}}}
\newcommand{\bP}{\mbox{\boldmath{$P$}}}
\newcommand{\bQ}{\mbox{\boldmath{$Q$}}}
\newcommand{\be}{\mbox{\boldmath{$e$}}}
\newcommand{\bE}{\mbox{\boldmath{$E$}}}
\newcommand{\bu}{\mbox{\boldmath{$u$}}}
\newcommand{\bx}{\mbox{\boldmath{$x$}}}
\newcommand{\bd}{\mbox{\boldmath{$d$}}}
\newcommand{\bxi}{\mbox{\boldmath{$\xi$}}}
\newcommand{\btu}{\tilde{\mbox{\boldmath{$u$}}}}
\newcommand{\bU}{\mbox{\boldmath{$U$}}}
\newcommand{\bv}{\mbox{\boldmath{$v$}}}
\newcommand{\bw}{\mbox{\boldmath{$w$}}}
\newcommand{\whk}{\mbox{{\boldmath $w$}$_n^{hk}$}}
\newcommand{\whkj}{\mbox{{\boldmath $w$}$_j^{hk}$}}
\newcommand{\whkjminus}{\mbox{{\boldmath $w$}$_{j-1}^{hk}$}}
\newcommand{\uhk}{\mbox{{\boldmath $u$}$_n^{hk}$}}
\newcommand{\uhkj}{\mbox{{\boldmath $u$}$_j^{hk}$}}
\newcommand{\uhkjminus}{\mbox{{\boldmath $u$}$_{j-1}^{hk}$}}
\newcommand{\xihk}{\mbox{{\boldmath $\xi$}$_n^{hk}$}}
\newcommand{\xihkj}{\mbox{{\boldmath $\xi$}$_j^{hk}$}}
\newcommand{\xihkjtau}{\xihkj_{\hspace{-.1cm}\tau}}
\newcommand{\bvs}{\mbox{\boldmath{\footnotesize$v$}}}
\newcommand{\btui}{\mbox{\boldmath{$\xi$}}}
\newcommand{\by}{\mbox{\boldmath{$y$}}}
\newcommand{\bz}{\mbox{\boldmath{$z$}}}
\newcommand{\bI}{\mbox{\boldmath{$I$}}}
\newcommand{\fb}{\mbox{\boldmath{$f$}}}
\newcommand{\fg}{\mbox{\boldmath{$g$}}}
\newcommand{\bsigma}{\mbox{\boldmath{$\sigma$}}}
\newcommand{\btau}{\mbox{\boldmath{$\tau$}}}
\newcommand{\bvarphi}{\mbox{\boldmath{$\varphi$}}}
\newcommand{\bvarepsilon}{\mbox{\boldmath{$\varepsilon$}}}
\newcommand{\bnu}{\mbox{\boldmath{$\nu$}}}
\newcommand{\beeta}{\mbox{\boldmath{$\eta$}}}
\newcommand{\bzeta}{\mbox{\boldmath{$\zeta$}}}
\newcommand{\bzero}{\mbox{\boldmath{$0$}}}
\newcommand{\bgamma}{\mbox{\boldmath{$\gamma$}}}
\newcommand{\blambda}{\mbox{\boldmath{$\lambda$}}}
\newcommand{\signu}{\mbox{\boldmath{${\sigma\nu}$}}}
\newcommand{\skalar}[1]{\left\langle #1 \right\rangle}
\newcommand{\sskalar}[1]{\langle\langle #1 \rangle\rangle}
\newcommand{\dual}[2]{\left\langle #1 \right\rangle_{{#2}^*\times #2}}
\newcommand{\ddual}[2]{\langle\langle #1 \rangle\rangle_{{#2}^*\times #2}}
\newcommand{\toweak}{\rightharpoonup}


% \newtheorem{Definicja}{Definicja}
% \newtheorem{Twierdzenie}{Twierdzenie}
% \newtheorem{Lemat}{Lemat}
% \newtheorem{Wniosek}{Wniosek}
